A Semi-Supervised Self-Organizing Map for Clustering and Classification

There has been an increasing interest in semi-supervised learning in the recent years because of the great number of datasets with a large number of unlabeled data but only a few labeled samples. Semi-supervised learning algorithms can work with both types of data, combining them to obtain better performance for both clustering and classification. Also, these datasets commonly have a high number of dimensions. This article presents a new semi-supervised method based on self-organizing maps (SOMs) for clustering and classification, called Semi-Supervised Self-Organizing Map (SS-SOM). The method can dynamically switch between supervised and unsupervised learning during the training according to the availability of the class labels for each pattern. Our results show that the SS-SOM outperforms other semi-supervised methods in conditions in which there is a low amount of labeled samples, also achieving good results when all samples are labeled.

==> algorithms/clustering.tex <==
\begin{algorithm}[!ht]
\ForEach{test input pattern \textbf{x}}
{
	Present \textbf{x} to the map;
    
	Compute the activation of all nodes (\eref{activation_dssom});
    
    Find the first winner $s_1$ with the highest activation ($a_s$) (\eref{winner_dssom});
    
    \eIf{$a_s \geq a_t$}
    { 
    	$s_f \gets s_1$;
        
    	\If{class($s_f$) = noClass}
        { 
        	Try to find a new winner $s_2$ with a define class and an activation above $a_{t}$;
    
    		\If{$s_2$ exists}
    		{
            	$s_f \gets s_2$;
        	}
        }
        
        Assign \textbf{x} to the cluster with the index of the winner node $s_f$;
        
        Set the predicted class of \textbf{x} to be the same class as the node represents (defined or undefined).
    } { 
    	Assign \textbf{x} to the outliers set;
    }
    
    
}
\caption{Clustering and Classification with SSH-SOM}
\label{alg:clustering}
\end{algorithm}

==> algorithms/convergence_phase.tex <==
\begin{algorithm}[!ht]

$\textit{N}_{max}$ $\gets$ \textit{N};

\While {nwins $<$ age\_wins}
{
    Choose a random input pattern \textbf{x};

	Compute the activation of all nodes (\eref{activation_dssom});

	Find the winner $s_1$ with the highest activation ($a_s$) (\eref{winner_dssom});
    
	\eIf{\text{\textbf{x} has a label}}
    { 
    	Run the Supervised Mode (\aref{alg:supervised-mode}) with \textbf{x} as input;
        
    } {
    	Run the Unsupervised Mode (\aref{alg:unsupervised-mode}) with \textbf{x} as input;
    }
    
    \If{\textit{nwins} = \textit{age\_wins}}
    {
    	Remove nodes with $wins_{j}$ $<$ \textit{lp} $\times$ \textit{age\_wins};
        
    	Update the connections of the remaining nodes as per \eref{update_neighborhood_larfdssom};
        
        Reset the number of wins of the remaining nodes:
        
        $wins_{j}$ $\gets$ 0;
        
        \textit{nwins} $\gets$ 0;
    }
    
    \textit{nwins} $\gets$ \textit{nwins} + 1;
}
nwins $\gets$ 0;

\caption{Convergence Phase}
\label{alg:convergence-phase}
\end{algorithm}
